Enabling All In-Edge Deep Learning: A Literature Review

In recent years, deep learning (DL) models have demonstrated remarkable achievements on non-trivial tasks such as speech recognition and natural language understanding. One of the significant contributors to its success is the proliferation of end devices that acted as a catalyst to provide data for data-hungry DL models. However, computing DL training and inference is the main challenge. Usually, central cloud servers are used for the computation, but it opens up other significant challenges, such as high latency, increased communication costs, and privacy concerns. To mitigate these drawbacks, considerable efforts have been made to push the processing of DL models to edge servers. Moreover, the confluence point of DL and edge has given rise to edge intelligence (EI). This survey paper focuses primarily on the fifth level of EI, called all in-edge level, where DL training and inference (deployment) are performed solely by edge servers. All in-edge is suitable when the end devices have low computing resources, e.g., Internet-of-Things, and other requirements such as latency and communication cost are important in mission-critical applications, e.g., health care. Firstly, this paper presents all in-edge computing architectures, including centralized, decentralized, and distributed. Secondly, this paper presents enabling technologies, such as model parallelism and split learning, which facilitate DL training and deployment at edge servers. Thirdly, model adaptation techniques based on model compression and conditional computation are described because the standard cloud-based DL deployment cannot be directly applied to all in-edge due to its limited computational resources. Fourthly, this paper discusses eleven key performance metrics to evaluate the performance of DL at all in-edge efficiently. Finally, several open research challenges in the area of all in-edge are presented.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

==> dat620-setup.tex <==
%DON'T CHANGE THIS FILE
%This file sets several properties for the ACM template.
%It is not necessary to change this file.


% Copyright
\setcopyright{none}

% DOI
\acmDOI{}

% ISBN
\acmISBN{}

%Conference
\acmConference[Project in Computer Science (DAT620)]{}{IDE}{UiS}
\acmBooktitle{}
\copyrightyear{2018}

\newcommand{\supervisors}[1]{\thanks{Supervised by #1}}


==> tex/abstract.tex <==
\textbf{This document serves both as a template and a guideline for your report. You can replace headings and body text with your content. Before you start writing, however, we recommend that you carefully consider the instructions in this document.
}

The abstract describes in concise words what you do, why you do it (not
necessarily in this order), and the main result. The abstract
has to be self-contained and readable for a person in the
general area. We suggest to write the abstract first,
as a means to guide the work, but it should be updated continuously.


==> tex/background.tex <==
Give a short, self-contained summary of necessary background
information. 

For our example if your project is a new \paxos implementation, the background
would be a brief introduction to the consensus problem, the \paxos algorithm,
the system model used by the \paxos algorithm
and common optimizations and relevant variations of that algorithm.

The goal of the background section is to make the paper 
self-contained for an audience as large as possible. As in every
section you start with a very brief overview of the section.
For our example that would be: In this section, we introduce the consensus problem,
the \paxos algorithm and common optimizations of that algorithm.

If you copy a definition from a text book or some other source, you must cite that source. 
See Example~\ref{def:consensus} below. 


==> tex/citations.tex <==
It is important that you correctly refer to sources. 

\begin{itemize}
\item If you describe background, according to some textbook, cite that textbook. \emph{See Example~\ref{def:consensus} below.}
\item If you make a claim about trends in industry or research, add citations to validate the claim. \emph{See Example~\ref{ex:trend} below.}
\item \textbf{Do not copy paste text from any source into your report without citation. It will be considered plagiarism.}
\item Always use the tilde character between the text and the cite command, e.g.:\begin{verbatim}
DBLP~\cite{dplg}
\end{verbatim}
The tilde inserts a space, but prevents line break between the text and citation.
\item For correct citations we recommend that you export bibtex entries from DBLP~\cite{dplg}. 
%@Hein: ACM produces crappy doi-urls for non ACM publications. I do believe that there are few papers that are part of the ACM-DL and not in DBLP.
But make sure to update the bibtex entries to adhere to the following rules.
\end{itemize}

Here are some rules to be followed for your bibliography:

\begin{itemize}
\item Make sure titles are correctly capitalized.

%You can export all nsdi citations from DBLP, accordingly this should not be a problem.
% \item Make sure abbreviations are consistent (e.g., is NSDI spelled out or
% not?) - using the @abbrev function in latex helps here.

\item Make sure there is enough info for a reader to find the document: authors
plus title isn't enough.

\item Don't blindly copy and paste ACM bibtex entries without fixing them:

- they list "New York, NY" as the address field, which means that all ACM
conferences look like they took place there; just delete this, or - better

- replace it with where the conference took place, which is much more
helpful to the reader than the publisher's address

- they have a truly weird idea about how to capitalize conference names;
just correct this (consistently)

* IEEE is equally bad, and uses a partially-inverted form of conference
names.

* Please actually review the bibliography before submitting your paper!
\end{itemize}

%@Leander: Move this to the Latex part:

And while you are at it, please:

\begin{itemize}
\item Add include{mathpmtc} in the main LaTeX file, so you don't have
math stuff in a different font than the main text. 
%We could simply add this to the template if not already done.

\item Always use the tilde character between the number and unit, e.g. 100~Mbps or 53~ms. 
The tilde inserts a space, but prevents line break between the number and unit.

\item Never put SI units in italics. 

\item Do differentiate between bits (b) and bytes (B), and between powers of 10~(MB) and 2~(MiB).

\item Avoid things like: "We refer the reader to [42]." That is, don't use citations as nouns.
\end{itemize}


\begin{example}
\label{def:consensus}
Consensus is a distributed programming abstraction that fulfills the following properties~\cite{aTextbook}:
\begin{description}
\item[Termination]
\item[Validity]
\item[Integrity]
\item[Agreement]
\end{description}
\end{example}

\noindent
\begin{example}
\label{ex:trend} Consensus systems build a fundamental part of todays cloud-computing infrastructure~\cite{spanner,chubby,zookeeper,zookeeperWeb}.
\end{example}



==> tex/conclusion.tex <==
Here you need to summarize what you did and why this is
important. Do not take the abstract and put it in the past
tense. Remember, now the reader has (hopefully) read the
paper, so it is a very different situation from the abstract.
Try to highlight important results and say the things you really
want to get across such as high-level statements (e.g.,
we believe that .... is the right approach to .... Even though
we only considered LAN, the .... technique should be applicable
....) You can also formulate next steps if you want.
Be brief.

==> tex/evaluation.tex <==
Here you evaluate your work using experiments. You start
again with a very short summary of the section. The typical
structure follows.

\subsection{Experimental setup}
Specify the context and setup of your experiments. This includes e.g.~what hardware (VMs) you are running on, what operating system these machines are running, how they are connected, ...

Also explain how you generate load for your system and what parameters you used here. The general idea is to include enough information for others to reproduce your experiments. To that end, you should provide a detailed set of instructions for repeating your experiments. These instructions should not be included in the report, but should be provided as part of the source code repository on GitHub, typically as the \texttt{README.md} file, or as Shell scripts or Ansible scripts.

If your experiments give strange or unexpected results, analyze, profile and debug your code. \textbf{Do not simply re-run experiments until they give the expected results.}

Finally, running experiments is very time consuming and you may need to go through multiple rounds of experiment, debugging and optimization. \textbf{Do not delay running experiments until the end of your project period.} 

\subsection{Results}
The results of your experiments. Compare different variants of your design (e.g.~with and without optimizations) or compare performance to other designs or systems. Plots should show the average over multiple runs (at least 10 as a rule of thumb), including error bars, percentiles or min/max values.

Discuss the plot and extract the overall performance. Do not repeat all numbers in the text, but mention relevant differences in numbers, e.g.~our optimization improves throughput by 26\%.
Discuss how the results validate or contradict your assumptions.

Perform experiments to evaluate your system under operating normal conditions, when experiencing failures or attacks, or with different workloads.

Figure~\ref{fig:graph} shows a graph generated with \texttt{pgfplots} from 
experiment data.
\begin{figure}
\begin{tikzpicture}
\begin{axis}[
    xlabel=Throughput ($\times 1000$ Ops/sec),
    ylabel=Latency (ms),
    legend entries={baseline, optimized},
]
%The mockup experiment data is stored in a csv file, and imported here.
\addplot table [x=throughput, y=latency, col sep=comma] {data/data-unoptimized.csv};
\addplot table [x=throughput, y=latency, col sep=comma] {data/data-optimized.csv};
\end{axis}
\end{tikzpicture}
\caption{A graph showing latency and throughput of a baseline and optimized implementation. The axes show latency in milliseconds, and throughput in thousand operations per second. Data is made up.}
\label{fig:graph}
\end{figure}


==> tex/further.tex <==
Here are some other useful resources: (make these into references instead of links?)
\begin{itemize}
\item The co-chairs of the Ninth SOSP prepared some recommendations and valuable lessons in a paper titled \textit{How (and How Not) to Write a Good Systems Paper} \url{https://www.usenix.org/legacy/publications/library/proceedings/dsl97/good_paper.html}
\item \url{http://gramoli.redbellyblockchain.io/web/doc/talks/researchmethod.pdf}
\item \url{https://www.doc.ic.ac.uk/~prp/doc/talks/11-prp-paper_writing.pdf}
\item This template is inspired by a template from Markus P\"uschel~\cite{puschel}.

\end{itemize}

==> tex/introduction.tex <==

\noindent
The introduction is different from the abstract; it should elaborate
more on the context of the work and other aspects. Generally, you can repeat some
of the main points also in the introduction, but expand and use different words.

To make your report easier to read, we recommend that you write in first person,
plural, i.e.~write \textit{we}, even if the report is single author.
This is also to represent that, even though you are writing this on your own,
your supervisor and possibly others are contributing ideas, suggestions and
corrections on your report.

What follows is a possible structure of the introduction.
Note that the structure can be modified, but the content should be the same.
Introduction and Abstract should fill at most the first page.

\paragraph{Context and Motivation} The first few sentences in the introduction
is typically a brief description providing context for your work, explaining
the broader domain of the work. This context should lead into the motivation for
the work by identifying one or more problems. 

Here is an example from~\cite{zorfu}:

\textit{Traditional desktop applications, such as word processing, email, and photo management are increasingly moving to server-based deployments. However, moving applications to the cloud can reduce availability because Internet path availability averages only two-nines~\cite{internetPaths}. If a user's application state is isolated on a single server, the availability for that user is limited by the path availability between the user's desktop and that server. Hence, to improve availability, application state must be replicated across multiple servers placed in geographically distributed data centers.}

\paragraph{Research Problem} This paragraph further restricts the problem introduced in the motivation to the problem you are addressing. 
Make sure to explain to the reader 
what you are doing, why it is important, and why it is non-trivial.

\paragraph{Related Work} Next, you have to give a brief overview
of related work. For a paper like this, anywhere between 2
and 8 references. Briefly explain what they do. End the paragraph by
contrasting their work to what you do, to make it precisely clear what
your contribution is.

\paragraph{Contribution Summary} 
It can be a good idea to end the introduction with a summary of your contributions as bullet points.
For example:
\begin{itemize}
\item We implement \paxos using brand new technologies.
\item We evaluate our implementation both in a WAN and LAN environment and show that it is $1.0001\times$ faster than state of the art.
\end{itemize}
It is not necessary to have a paragraph at the end of the introduction, that lists the following sections. 


==> tex/latex.tex <==
This section contains some instructions and examples for using \LaTeX.

\subsection{You can add subsections}
You can use numbered subsections to structure your sections or $\backslash\texttt{paragraph}$ to separate paragraphs with a heading using only a few words, as used in Section~\ref{sec:introduction}.


\begin{enumerate}
	\item\label{item:1} This is an item in an enumeration.
    \begin{itemize}
    	\item This is an item of a unnumbered list. In this case, the lists are nested within each other.
    \end{itemize}
    \item\label{item:2} The second point in the enumerated list.
\end{enumerate}
%
I can refer to the element of the enumeration above as Point~\ref{item:1}.
If you refer to numbered items,~e.g. items from a list or figures or sections, always capitalize the name. 
For example, this is Section~\ref{sec:latex}.

\subsection{Figures}
You can include figures. You can include files, as done in Figure~\ref{fig:example}. 
Avoid including jpeg, gif or bmp files since these do not scale nicely. Again Figure~\ref{fig:example} is an example for that.

\begin{figure}[t]
   \centering
   \includegraphics[width=\linewidth]{fig/RegisterOperations}
    \caption{Figure taken from~\cite{lecture}}
    \label{fig:example}
\end{figure}

You can create graphs from your experiment-data using \texttt{pgfplots}.
See the example in \texttt{tex/evaluation.tex} and documentation \url{http://pgfplots.sourceforge.net/pgfplots.pdf}.

\subsection{Other tips}
\begin{itemize}

\item Always use the tilde character between the number and unit, e.g. 100~Mbps or 53~ms. The tilde inserts a space, but prevents line break between the number and unit.

\item Never put SI units in italics. 

\item Do differentiate between bits (b) and bytes (B), and between powers of 10~(MB) and 2~(MiB).

\item Avoid things like: "We refer the reader to [42]." That is, don't use citations as nouns.
\end{itemize}

For further instructions on how to add \textbf{Tables, Algorithms, Theorems see acmguide.pdf}.


==> tex/method.tex <==
Now comes the "beef" of the paper, where you explain what
you did. Again, organize it in paragraphs with titles. As in
every section you start with a very brief overview of the
section. 

This section may vary significantly depending on your topic.
You may also choose to make the different parts individual sections.
Here is a more general structure:

\subsection{Design} Concisely present your design. Focus on novel aspects,
but avoid implementation details. Use pseudo-code and figures to better
explain your design, but also present and explain these in the text.
%
To assist in evaluating your design choices, it may be relevant to describe
several distinct \textit{design alternatives} that can later be compared.

\subsection{Analysis} Argue for the correctness of your design and 
why you expect it to perform better than previous work.
%
If applicable, mention how your design relates to theoretical bounds.

\subsection{Optimization} Explain how you optimized your design and 
adjusted it to specific situations.
%
Generally, as important as the final results is to show
that you took a structured, organized approach to the optimization
and that you explain why you did what you did.
%
Be careful to argue, why your optimization does not break the 
correctness of your design, established above.
%
It is often a good strategy to explain a design or protocol in stepwise refinements,
so as to more easily convince the reader of its correctness. 

\subsection{Implementation} It is not necessary to "explain" your code. 
However, in some cases it may be relevant to highlight 
additional contributions given by your implementation.
Examples for such contributions are:
\begin{itemize}
\item \emph{Abstractions and modules}: If your implementation is nicely separated into interacting
modules with separated responsibilities you could explain this structure,
and why it is good/better than some other alternative structure.
\item \emph{Optimization}: If you spend significant time optimizing your code, e.g.~using profiling tools,
the result of such optimization may be presented as a contribution. In this case, reason, 
why the optimized code works better.
\item \emph{Evaluation framework}: If you implemented a framework or application to evaluate your implementation against existing work, or in a specific scenario, this framework may be presented as a contribution.
\end{itemize}

Make sure to cite all external resources used.

